An Efficient Algorithm for Classical Density Functional Theory in Three Dimensions: Ionic Solutions

Classical density functional theory (DFT) of fluids is a valuable tool to analyze inhomogeneous fluids. However, few numerical solution algorithms for three-dimensional systems exist. Here we present an efficient numerical scheme for fluids of charged, hard spheres that uses $\mathcal{O}(N\log N)$ operations and $\mathcal{O}(N)$ memory, where $N$ is the number of grid points. This system-size scaling is significant because of the very large $N$ required for three-dimensional systems. The algorithm uses fast Fourier transforms (FFT) to evaluate the convolutions of the DFT Euler-Lagrange equations and Picard (iterative substitution) iteration with line search to solve the equations. The pros and cons of this FFT/Picard technique are compared to those of alternative solution methods that use real-space integration of the convolutions instead of FFTs and Newton iteration instead of Picard. For the hard-sphere DFT we use Fundamental Measure Theory. For the electrostatic DFT we present two algorithms. One is for the \textquotedblleft bulk-fluid\textquotedblright functional of Rosenfeld [Y. Rosenfeld. \textit{J. Chem. Phys.} 98, 8126 (1993)] that uses $\mathcal{O}(N\log N)$ operations. The other is for the \textquotedblleft reference fluid density\textquotedblright (RFD) functional [D. Gillespie et al., J. Phys.: Condens. Matter 14, 12129 (2002)]. This functional is significantly more accurate than the bulk-fluid functional, but the RFD algorithm requires $\mathcal{O}(N^{2})$ operations.

==> Writeup-Confined.tex <==
\section{Confined Ions}

    Confined ions are restricted to a certain subset of the domain. For example, charged terminal groups of aspartates
tethered to the wall of an ion channel may be modeled in this fashion. However, since we fix the number of ions rather
than an electrochemical potential, we determine an effective potential $\mu^{eff}$ for this species using an explicit
integral. For a confined species $i$, we express their density $\rho_i$ as
\begin{equation}
  \rho_i = \exp\left\{\mu^{eff}_i - \mu^{ext}_i - \mu^{HS}_i - \mu^{SC}_i - z_i e \phi \right\}.
\end{equation}
with the unknown effective electrochemical potential $\mu^{eff}_k$. We can now impose an integral constraint, fixing the
number of ions $N_k$,
\begin{eqnarray}
  N_i &=& \int \rho_i d^3x \\
      &=& \int exp\left\{\mu^{eff}_i - \mu^{ext}_i - \mu^{HS}_i - \mu^{SC}_i - z_i e \phi \right\} d^3x \\
      &=& e^{\mu^{eff}_i} \int exp\left\{-\mu^{ext}_i - \mu^{HS}_i - \mu^{SC}_i - z_i e \phi \right\} d^3x
\end{eqnarray}
so that
\begin{equation}
  \mu^{eff}_i = \log N_k - \log\left(\int exp\left\{-\mu^{ext}_i - \mu^{HS}_i - \mu^{SC}_i - z_i e \phi \right\}\right),
\end{equation}

In the code, we use this to define an effective concentration
\begin{equation}
  \rho^{eff}_i = \frac{N_i}{\int exp\left\{-\mu^{ext}_i - \mu^{HS}_i  - \mu^{SC}_i - z_i e \phi \right\}},
\end{equation}
which mimics the role of the ionic bath concentration in our residual calculation, and is recalculated at each residual
evaluation. We choose $\mu^{ext}_i$ to confine these ions to the selectivity filter. In our examples, the barrier at the
filter ends are hard walls, but need not be and could ramp up over a few angstroms.

